Speakable in quantum mechanics: babbling on

This paper consists of a short version of the derivation of the intuitionistic quantum logic L_QM (which was originally introduced by Caspers, Heunen, Landsman and Spitters). The elaboration consists of extending this logic to a classical logic CL_QM. Some first steps are then taken towards setting up a probabilistic framework based on CL_QM in terms of R\'enyi's conditional probability spaces. Comparisons are then made with the traditional framework for quantum probabilities.

==> eptcsdata.tex <==
\providecommand{\firstpage}{53}
\providecommand{\publicationstatus}{R. Duncan and P. Panangaden (Eds.)\\
Quantum Physics and Logic 2012 (QPL2012)\\
EPTCS 158, 2014, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.158.5}{10.4204/EPTCS.158.5}}

